Teachers Do More Than Teach: Compressing Image-to-Image Models

Generative Adversarial Networks (GANs) have achieved huge success in generating high-fidelity images, however, they suffer from low efficiency due to tremendous computational cost and bulky memory usage. Recent efforts on compression GANs show noticeable progress in obtaining smaller generators by sacrificing image quality or involving a time-consuming searching process. In this work, we aim to address these issues by introducing a teacher network that provides a search space in which efficient network architectures can be found, in addition to performing knowledge distillation. First, we revisit the search space of generative models, introducing an inception-based residual block into generators. Second, to achieve target computation cost, we propose a one-step pruning algorithm that searches a student architecture from the teacher model and substantially reduces searching cost. It requires no l1 sparsity regularization and its associated hyper-parameters, simplifying the training procedure. Finally, we propose to distill knowledge through maximizing feature similarity between teacher and student via an index named Global Kernel Alignment (GKA). Our compressed networks achieve similar or even better image fidelity (FID, mIoU) than the original models with much-reduced computational cost, e.g., MACs. Code will be released at https://github.com/snap-research/CAT.

==> figs/fig_img_results.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{./imgs/placeholder.png}
\caption{\todo{Show some images, CylcleGAN, Pix2Pix, GauGAN, and Clade.}}\label{fig:img_results}
\end{figure*}

==> figs/fig_pipeline.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.9\linewidth]{./imgs/pipeline.pdf}
\caption{\todo{Pipeline. Content in the figure: Overall pipeline (pruning, cka), searching space design}}\label{fig:pipeline}
\end{figure}

==> figs/fig_spade_original.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=.9\linewidth]{./imgs/spade.pdf}
\caption{SPADE normalization module where the input is utilized to determine the scaling and shifting parameters for batch normalization.}\label{fig:spade_original}
\end{figure}

==> figs/fig_supp_cityscape.tex <==
\begin{figure*}[]
\centering
%\includegraphics[width=1\linewidth]{./imgs/cityscapes-4-dark.pdf}
\caption{
Additional results on Cityscapes dataset with Pix2pix model.
}
\label{fig:supp_city}
\end{figure*}

==> figs/fig_supp_zebra.tex <==
\begin{figure*}[]
\centering
\includegraphics[width=.61\linewidth]{./imgs/zebra_additional.pdf}
\caption{
Results on Zebra$\shortrightarrow$Horse dataset. Compared with original CycleGAN, our model has much reduced MACs and can generate images with higher fidelity (lower FID).}
\label{fig:supp_zebra}
\end{figure*}

==> tabs/tab_atomnas_hyper.tex <==
\begin{table}[h]
    \centering
    \caption{Analysis of the hyperparmeters of atomnas on Cityscape. \textcolor{red}{The goal is to show that atomnas (iterative pruning) is hyperparameters sensitive, and we put lots of efforts to find the best hyperparameters.}}
    \label{tab:hyper_analysisi}
    \begin{tabular}{c|ccc}
        \toprule
        Method & $\lambda$ & prune per epoch & mIoU$\uparrow$  \\ \midrule
        Atomnas  \\
        Atomnas  \\
        Atomnas  \\ \bottomrule
    \end{tabular}
\end{table}

==> tabs/tab_clade.tex <==
\begin{table*}[h]
    \centering
    \caption{Quantitative comparison between different techniques for Image-to-Image models on Cityscapes dataset.
    We use FID to evaluate the generation quality.
    Lower FID indicates better performance.
    }
    \label{tab:clade}
    \begin{tabular}{lclccc}
        \toprule
    Model & Method & MACs & FID$\downarrow$ \\ \midrule
        % ======= numbers for gaugan
        GauGAN & Park~\etal~\cite{park2019semantic} &  281\fu  & 55.15 \\
        % ======= numbers for clade
        Clade & Tan~\etal~\cite{tan2020rethinking} & 75.2\fu & 55.81 \\
        Clade-Avg & \textbf{Ours} & \textbf{75.2\fu}  & \textbf{54.52}
        \\\bottomrule
    \end{tabular}
\end{table*}

==> tabs/tab_gaugan_flops.tex <==
\begin{table}[h]
    \centering
    \caption{Computational cost comparison between Pix2Pix and GauGAN.}
    \label{tab:gaugan_flops}
    \begin{tabular}{lc}
    \toprule
    Model & MACs \\ \midrule
    Pix2Pix & 56.8\fu \\ GauGAN & 281\fu 
    \\\bottomrule
    \end{tabular}
\end{table}

==> tabs/tab_l1_norm.tex <==
\begin{table}[h]
    \centering
    \caption{Analysis of L1 norm on Cityspace for Pix2pix (\textcolor{red}{Discussion Only}).}
    \label{tab:l1}
    \begin{tabular}{l|c|c}
        \toprule
        L1 & Normalized & mIoU$\uparrow$  \\ \midrule
        0 & - & $35.46_{}$ \\
        1e-4 & N & $35.05_{}$ \\
        1e-3 & N & $34.07_{}$ \\
        1e-2 & N & $34.29_{}$ \\
        1e-1 & N & $32.91_{}$ \\
        1 & N & $35.23_{}$ \\
        1e-4 & Y & $35.05_{}$ \\
        1e-3 & Y & $34.07_{}$ \\
        1e-2 & Y & $34.29_{}$ \\
        1e-1 & Y & $32.91_{}$ \\
        1 & Y & $35.23_{}$ \\
        \bottomrule
    \end{tabular}
\end{table}




\iffalse

\begin{table}[h]
    \centering
    \caption{Analysis of L1 norm on Cityspace for Pix2pix (\textcolor{red}{Discussion Only}).}
    \label{tab:l1}
    \begin{tabular}{l|c|c}
        \toprule
        L1 & Normalized & mIoU$\uparrow$  \\ \midrule
        0 & - & 35.46 \\
        1e-4 & N & 35.05 \\
        1e-3 & N & 34.07 \\
        1e-2 & N & 34.29 \\
        1e-1 & N & 32.91 \\
        0.05 & Y & 35.23 \\
        0.1 & Y & 35.06 \\
        0.5 & Y & 32.27 \\
        1.0 & Y & 34.53 \\
        \bottomrule
    \end{tabular}
\end{table}


resnet\_9block, pix2pix, cityscapes (for discussion only)
-----------------------
l1      norm     mIoU
0       -        35.46
1e-4    N        35.05
1e-3    N        34.07
1e-2    N        34.29
1e-1    N        32.91
0.05    Y        35.23
0.1     Y        35.06
0.5     Y        32.27
1.0     Y        34.53
-----------------------

\begin{table}[h]
    \centering
    \caption{Analysis of L1 norm on Cityspace for Pix2pix.}
    \label{tab:distillation}
    \begin{tabular}{l|cc}
        \toprule
        Method & MACs & mIoU$\uparrow$  \\ \midrule
        Teacher & 11.4B & 45.89 \\
        Teacher + L1 & xx & xx \\
        \bottomrule
    \end{tabular}
\end{table}

Our original purpose is to demonstrate that, although L1 is helpful for model sparsification and compression, it harms the performance. We need to prove that for L1 penalty that helps sparsification, it harms the performance.

\fi




\iffalse

\begin{table}[h]
    \centering
    \caption{Analysis of L1 norm on Cityspace for Pix2pix.}
    \label{tab:distillation}
    \begin{tabular}{l|cc}
        \toprule
        Method & MACs & mIoU$\uparrow$  \\ \midrule
        Coarse Pruning Only (Baseline) & 11.4B & 45.89 \\
        Coarse Pruning + L1 & xx & xx \\
        Coarse Pruning + L1 renorm & 11.4B & 41.94 \\\midrule
        Coarse Pruning + L1 pruning & 5.58B & 38.22 \\
        Coarse Pruning + L1 pruning + ft & 5.58B & \textcolor{blue}{\bf 43.16} \\
        Coarse Pruning + L1 renorm pruning & 5.48B & 41.13 \\
        %Baseline + L1 renorm pruning + ft & xx & xx \\
        \bottomrule
    \end{tabular}
\end{table}

\fi
